StrobeNet: Category-Level Multiview Reconstruction of Articulated Objects

We present StrobeNet, a method for category-level 3D reconstruction of articulating objects from one or more unposed RGB images. Reconstructing general articulating object categories % has important applications, but is challenging since objects can have wide variation in shape, articulation, appearance and topology. We address this by building on the idea of category-level articulation canonicalization -- mapping observations to a canonical articulation which enables correspondence-free multiview aggregation. Our end-to-end trainable neural network estimates feature-enriched canonical 3D point clouds, articulation joints, and part segmentation from one or more unposed images of an object. These intermediate estimates are used to generate a final implicit 3D reconstruction.Our approach reconstructs objects even when they are observed in different articulations in images with large baselines, and animation of reconstructed shapes. Quantitative and qualitative evaluations on different object categories show that our method is able to achieve high reconstruction accuracy, especially as more views are added.

==> tables/ablation_NAOCS.tex <==
\renewcommand{\arraystretch}{1}
\setlength{\tabcolsep}{5pt}
\begin{table*}[th!]
\centering
% \vspace{0pt}
\centering
\footnotesize
\resizebox{1\linewidth}{!}{
% \resizebox{0.98\linewidth}{!}{
\begin{tabular}{lcccccccc|cc}
    \toprule
    \textbf{Class}     & \multicolumn{2}{c}{\textbf{eyeglasses}} &  \multicolumn{2}{c}{\textbf{laptop}} &  \multicolumn{2}{c}{\textbf{oven}}    &
    \multicolumn{2}{c}{\textbf{chair}}    &
    \multicolumn{2}{c}{\textbf{mean}}\\    

    \textbf{Metric}   & \textbf{CD~$\downarrow$} & \textbf{IoU~$\uparrow$} & \textbf{CD~$\downarrow$} & \textbf{IoU~$\uparrow$} & \textbf{CD~$\downarrow$} & \textbf{IoU~$\uparrow$} &
    \textbf{CD~$\downarrow$} & \textbf{IoU~$\uparrow$}
    &
    \textbf{CD~$\downarrow$} & \textbf{IoU~$\uparrow$}
    \\
    \midrule
    \textbf{Ours} & \textbf{1.59$\pm$0.60 }  & \textbf{31.59$\pm$8.33} & \textbf{0.77 $\pm$ 0.21} & \textbf{64.94 $\pm$ 11.73} & \textbf{1.40 $\pm$ 0.41} & \textbf{67.98 $\pm$ 11.46} & \textbf{2.25 $\pm$ 0.85} & \textbf{31.96 $\pm$ 10.95} & \textbf{1.50} & \textbf{49.12} \\
    
    \textbf{w/o reposing} & 2.03$\pm$ 0.66 & 29.10$\pm$ 10.29 & 1.69 $\pm$ 0.42 & 59.73 $\pm$ 9.69  &  3.43  $\pm$ 1.13 & 56.83  $\pm$ 13.83 & 2.31 $\pm$ 0.95 & 26.82 $\pm$ 12.16 & 2.37 & 43.12 \\
    
    \bottomrule \\
  \end{tabular}

}
\caption{{\small An additional ablation experiments on the reposing operation. The first row shows the results by estimating NOCS in input pose and then repose it into pose canonical status(reposing from NOCS to NAOCS) and the second is by directly predicting NAOCS, in comparison, the reposing operation constantly and significantly improved the quality of reconstruction. }}
\label{tab:ablation_naocs}
\end{table*}

==> tables/ablation_expt.tex <==
\renewcommand{\arraystretch}{1}
\setlength{\tabcolsep}{5pt}
\begin{table}[t!]
\centering
% \vspace{0pt}
\centering
\footnotesize
\resizebox{0.5\linewidth}{!}{
% \resizebox{0.98\linewidth}{!}{
% \begin{tabular}{lcccccc|cc}
%     \toprule
%     \textbf{Class}     & \multicolumn{2}{c}{\textbf{eyeglasses}} &  \multicolumn{2}{c}{\textbf{laptop}} &  \multicolumn{2}{c}{\textbf{oven}}    & \multicolumn{2}{c}{\textbf{mean}}\\    

%     \textbf{Metric}   & \textbf{CD~$\downarrow$} & \textbf{IoU~$\uparrow$} & \textbf{CD~$\downarrow$} & \textbf{IoU~$\uparrow$} & \textbf{CD~$\downarrow$} & \textbf{IoU~$\uparrow$} &
%     \textbf{CD~$\downarrow$} & \textbf{IoU~$\uparrow$}\\
%     \midrule
%     \textbf{Ours} & \textbf{1.81 $\pm$ 0.89 }  & \textbf{31.7 $\pm$ 8.4 } & 0.86 $\pm$ 0.23 & \textbf{63.0 $\pm$ 9.8} & 1.25 $\pm$ 0.28& \textbf{67.8 $\pm$ 11.5 } & \textbf{1.31} & \textbf{54.1}  \\
%     \textbf{w/o consistency} & 2.44 $\pm$ 1.23 &  29.4 $\pm$ 9.7 & 0.86 $\pm$ 0.19 &  62.7 $\pm$ 8.7 & 1.39 $\pm$ 0.36 &  63.4 $\pm$ 7.4 & 1.56 & 51.8  \\
%     \textbf{w/o local feature} & 6.40 $\pm$ 3.80 &  24.0 $\pm$ 10.0 & \textbf{0.85 $\pm$ 0.24} &  61.6$ \pm$ 11.3 & \textbf{1.21 $\pm$ 0.34} & 65.8 $\pm$ 10.5 & 2.82 & 50.4  \\
%     % \textbf{Ours (multi-pose)} & 23.8/2.69 & 51.1/1.50 & \textbf{62.9}/1.80 & / \\
%     \bottomrule \\
%   \end{tabular}
\begin{tabular}{lcc}
    \toprule
     \multicolumn{3}{c}{\textbf{Mean performance}}\\    
    \textbf{Metric}   & \textbf{CD~$\downarrow$} & \textbf{IoU~$\uparrow$}\\
    \midrule
    \textbf{Ours} & \textbf{1.31} & \textbf{54.1}  \\
    \textbf{w/o consistency} & 1.56 & 51.8  \\
    \textbf{w/o local feature} & 2.82 & 50.4  \\
    % \textbf{Ours (multi-pose)} & 23.8/2.69 & 51.1/1.50 & \textbf{62.9}/1.80 & / \\
    \bottomrule \\
  \end{tabular}
  }
\caption{{\small Our ablation on two pipeline ingredient: consistency loss and local features, shows their effectiveness in improving overall reconstruction accuracy. Per-category results are provided in the supplementary. }}
\label{tab:ablation}
\end{table}

==> tables/arbitrary_view.tex <==
\renewcommand{\arraystretch}{1}
\setlength{\tabcolsep}{5pt}
\begin{table*}[t!]
\centering
% \vspace{0pt}
\centering
\footnotesize
\resizebox{\linewidth}{!}{
% \resizebox{0.98\linewidth}{!}{
\begin{tabular}{lcccccc|cc}
    \toprule
    \textbf{Class}     & \multicolumn{2}{c}{\textbf{eyeglasses}} &  \multicolumn{2}{c}{\textbf{laptop}} &  \multicolumn{2}{c}{\textbf{oven}}    & \multicolumn{2}{c}{\textbf{mean}}\\    

    \textbf{Metric}   & \textbf{CD~$\downarrow$} & \textbf{IoU~$\uparrow$} & \textbf{CD~$\downarrow$} & \textbf{IoU~$\uparrow$} & \textbf{CD~$\downarrow$} & \textbf{IoU~$\uparrow$} &
    \textbf{CD~$\downarrow$} & \textbf{IoU~$\uparrow$}\\
    \midrule
    \textbf{2-views} & 1.81 $\pm$ 0.89  & 31.7 $\pm$ 8.4 & 0.86 $\pm$ 0.23 & 63.0 $\pm$ 9.8 & 1.25 $\pm$ 0.28 & 67.8 $\pm$ 11.5 & 1.31 & 54.1 \\
    % \textbf{3-views} & 1.44 $\pm$ 0.62 &  36.2 $\pm$ 7.7 &  &  &  & &  &   \\
    \textbf{3-views} & 1.44 $\pm$ 0.62 &  36.2 $\pm$ 7.7 &  &  &  & &  &   \\
    \textbf{4-views} & 1.30 $\pm$ 0.52 &  37.5 $\pm$ 7.2 &  &  &  &  &  &   \\
    \textbf{5-views} & 1.21 $\pm$ 0.44 &  38.3 $\pm$ 6.9 &  &  &  &  &  &   \\
    \textbf{6-views} & 1.15 $\pm$ 0.40 &  38.6 $\pm$ 7.2 &  &  &  &  &  &   \\
    \textbf{7-views} & 1.12 $\pm$ 0.37 &  38.7 $\pm$ 7.1 &  &  &  &  &  &   \\
    \textbf{8-views} & 1.10 $\pm$ 0.34 &  38.6 $\pm$ 7.1 & 0.73 $\pm$ 0.28 & 66.6 $\pm$ 10.8 & 1.11 $\pm$ 0.29 & 71.7 $\pm$ 8.5 &  &   \\
    % \textbf{Ours (multi-pose)} & 23.8/2.69 & 51.1/1.50 & \textbf{62.9}/1.80 & / \\
    \bottomrule \\
  \end{tabular}

}
\caption{{\small Our experiments for arbitrary input view points, shows the performance imporoves consistently as the number of input views increase}}
\label{tab:arbitrary}
\end{table*}

==> tables/chair_results.tex <==
\renewcommand{\arraystretch}{1}
\setlength{\tabcolsep}{5pt}
\begin{table*}[th!]
\centering
% \vspace{0pt}
\centering
\footnotesize
\resizebox{0.6\linewidth}{!}{
% \resizebox{0.98\linewidth}{!}{
\begin{tabular}{lccccccc}
    \toprule
    \textbf{Method}     & \multicolumn{1}{c}{\textbf{Ours}} &  \multicolumn{1}{c}{\textbf{w/o consistency}} &  \multicolumn{1}{c}{\textbf{w/o local feature}}    & 
    % \multicolumn{1}{c}{\textbf{w/o 
    % repose}}  &
    \multicolumn{1}{c}{\textbf{OccNet-C}} \\
    \midrule
    \textbf{CD~$\downarrow$} & \textbf{2.25 $\pm$ 0.85}  & 2.32 $\pm$0.87 & 2.34 $\pm$ 0.86 & 4.05 $\pm$ 1.42 &   \\
    \textbf{IoU~$\uparrow$} & \textbf{31.96 $\pm$ 10.95} & 26.92 $\pm$ 8.44 & 30.94 $\pm$10.17 & 14.33 $\pm$ 8.40 &\\
    
    \bottomrule \\
  \end{tabular}
}
\caption{{\small Quantitative results on folding chairs. The first column is the result of StrobeNet, 2nd and 3rd columns shows results of basic ablation experiments, where our choice for the pipeline improved the performance as expected. The 4th column is a comparison to the OccNet\cite{OccNet} baseline, our method performed significantly better than it.}}
\label{tab:chair_results}
\end{table*}

==> tables/discarded/reconstructions_nobg.tex <==
\renewcommand{\arraystretch}{1.4}
\setlength{\tabcolsep}{5pt}
\begin{table*}[t!]
\centering
\vspace{0pt}
\centering
\footnotesize
% \usepackage{math}
\resizebox{1\linewidth}{!}{
% \resizebox{0.98\linewidth}{!}{
\begin{tabular}{llcccccc|cc}
    \toprule
    &\textbf{Class} & \multicolumn{2}{c}{\textbf{eyeglasses}} &  \multicolumn{2}{c}{\textbf{laptop}} &  \multicolumn{2}{c}{\textbf{oven}}    & \textbf{mean}\\    
    % \cline{2-5}
    &\textbf{Metric} & \textbf{CD~$\downarrow$} & \textbf{IoU~$\uparrow$} & \textbf{CD~$\downarrow$} & \textbf{IoU~$\uparrow$} & \textbf{CD~$\downarrow$} & \textbf{IoU~$\uparrow$} \\
    \midrule
    % chamfer dis - 0.048116 std 0.033175 -  IoU - 0.248093 std 0.111224
    % chamfer dis - 0.077236 std 0.063797 -  IoU - 0.250197 std 0.142996
    \multirow{2}{*}{\textbf{Single view}}&\textbf{OccNet-C}  &  16.20 $\pm$ 9.66 & 15.5 $\pm$ 14.8 & 1.49 $\pm$ 0.31 & 57.4 $\pm$ 9.27 & 2.45 $\pm$ 0.61 & 52.2 $\pm$ 13.0 & &  \\
    &\textbf{\ShortName} & \textbf{13.12 $\pm$ 5.12} & \textbf{16.5 $\pm$ 9.1} &  \textbf{1.41 $\pm$ 0.21} & \textbf{56.7 $\pm$ 11.3} & \textbf{1.50 $\pm$ 0.23} & \textbf{53.9 $\pm$ 12.9} & &  \\    
    \hline
    \multirow{2}{*}{\textbf{2 views}}&\textbf{OccNet-C} & 4.77 $\pm$ 5.76 & 27.8 $\pm$ 16.4 & 1.49 $\pm$ 0.57 & 52.7 $\pm$ 19.9 & 2.31 $\pm$ 0.64 & 57.4 $\pm$ 9.8 & / \\
    &\textbf{\ShortName}&\textbf{ 2.11 $\pm$ 0.96} & \textbf{32.5 $\pm$ 9.52} & \textbf{1.27 $\pm$ 0.27} & \textbf{59.0 $\pm$ 11.2}  & \textbf{1.76 $\pm$ 0.43} & \textbf{68.4 $\pm$ 11.2}  & &  \\
    \hline
    \multirow{2}{*}{\textbf{4 views}}&\textbf{OccNet-C} & 4.45  $\pm$ 3.04 & 24.6 $\pm$ 13.5 & 1.46 $\pm$ 0.22 & 59.5 $\pm$ 4.8 & 2.41 $\pm$ 0.51 & 52.0 $\pm$ 12.3 & &  \\
    
    &\textbf{\ShortName} & \textbf{2.32 $\pm$ 1.14} & \textbf{33.4 $\pm$ 7.86} & \textbf{1.06 $\pm$ 0.1} & \textbf{65.5 $\pm$ 7.0} & \textbf{1.62 $\pm$ 0.47} & \textbf{69.4 $\pm$ 12.0} & &  \\
    \bottomrule \\
  \end{tabular}}
\caption{\small{\textbf{Articulation-canonical} shape reconstruction from different number of input views. Our \ShortName consistently outperforms an OccNet\cite{OccNet}-based baseline in both CD and IoU.}}
\label{tab:compare}
%\vspace{-0.7cm}
\end{table*}

% sv_occ chamfer dis - 0.042640 std 0.026512 -  IoU - 0.236522 std 0.114761
% 


% \textbf{Ours (w/o consistency loss)} & 32.5/3.12 & 58.7/1.28 & 57.3/1.77 & /  \\
    % \textbf{Ours (w/o local feature)} & 26.6/8.66 & 62.1/11.4 & 61.3/1.60 & /  \\
    % \textbf{Ours (multi-pose)} & 23.8/2.69 & 51.1/1.50 & \textbf{62.9}/1.80 & / \\
    % chamfer dis - 0.011524 std 0.001843 -  IoU - 0.615534 std 0.083206
    % chamfer dis - 0.015556 std 0.003922 -  IoU - 0.711482 std 0.12630
    %  chamfer dis - 0.016257 std 0.004793 -  IoU - 0.693556 std 0.119950 oss is 0.10017
    % chamfer dis - 0.010671 std 0.001738 -  IoU - 0.655520 std 0.069587




% sep pose:  chamfer dis - 0.040137 std 0.020567 -  IoU - 0.227214 std 0.084271


==> tables/recon_input_pose_compact.tex <==
\renewcommand{\arraystretch}{1.4}
\setlength{\tabcolsep}{5pt}
\begin{table}[t!]
\centering
% \vspace{0pt}
\centering
\footnotesize
% \usepackage{math}
\resizebox{0.9\linewidth}{!}{
% \resizebox{0.98\linewidth}{!}{
\begin{tabular}{lccc|c}
    \toprule
    \textbf{Class} & {\textbf{eyeglasses}} &  {\textbf{laptop}} &  {\textbf{oven}}  &  {\textbf{mean}}\\    
    % \cline{2-5}
    \textbf{Metric} & \textbf{CD~$\downarrow$}/\textbf{IoU~$\uparrow$} & \textbf{CD~$\downarrow$}/\textbf{IoU~$\uparrow$} & \textbf{CD~$\downarrow$}/\textbf{IoU~$\uparrow$} & \textbf{CD~$\downarrow$}/\textbf{IoU~$\uparrow$}\\
    \midrule
    
    \textbf{OccNet-F} & 9.08/\textbf{24.12} &  1.51/51.69 & 4.31/51.64 & 4.96/42.48 \\
    
    \textbf{\ShortName} & \textbf{2.78}/21.98 & \textbf{1.12}/\textbf{54.91} & \textbf{2.01}/\textbf{61.83} & \textbf{1.97}/ \textbf{46.24} \\
    \hline
    
    % \multirow{2}{*}{\textbf{2 views}}&\textbf{OccNet-F} & 8.49 $\pm$ 2.37 & \textbf{27.77 $\pm$ 8.59} & 1.75 $\pm$ 0.47 & 45.77 $\pm$ 9.58 & 4.82 $\pm$ 1.78 & 50.25 $\pm$ 10.36 & 5.02 & 41.26 \\
    
    % &\textbf{\ShortName}& \textbf{2.16 $\pm$ 0.81} & 21.26 $\pm$ 8.83 & \textbf{1.23 $\pm$ 0.52} & \textbf{50.71 $\pm$ 11.96}  & \textbf{1.95 $\pm$ 0.89}& \textbf{60.86 $\pm$ 8.87}  & \textbf{1.78} & \textbf{44.28} \\
    % \hline
    
    % \multirow{2}{*}{\textbf{4 views}}&\textbf{OccNet-F} & 9.10 $\pm$ 2.69 & 28.20 $\pm$ 10.09 & 1.36 $\pm$ 0.30 & 56.98 $\pm$ 7.88 & 3.13 $\pm$ 1.21 & 52.95 $\pm$ 10.41 &  4.53 & 46.04 \\
    
    % &\textbf{\ShortName} & \textbf{2.00 $\pm$ 0.74} & \textbf{31.13 $\pm$ 8.50} & \textbf{1.06 $\pm$ 0.34} & \textbf{57.85 $\pm$ 10.34} & \textbf{1.95 $\pm$ 0.67} & \textbf{63.31 $\pm$ 8.15} & \textbf{1.67} & \textbf{50.76} \\
    \bottomrule \\
  \end{tabular}}
\caption{\small{\textbf{Reconstruction in Input Shape} shape reconstruction averaged over different number of input views. In most cases Our \ShortName outperforms an OccNet\cite{OccNet}-based baseline in both CD and IoU. An analysis for the failure on eyeglasses' IoU could be found in the supplemental.}}
\label{tab:input_pose}
%\vspace{-0.7cm}
\end{table}

==> tables/reconstruction_wtbg.tex <==
\renewcommand{\arraystretch}{1.4}
\setlength{\tabcolsep}{5pt}
\begin{table*}[t!]
\centering
% \vspace{0pt}
\centering
\footnotesize
\resizebox{0.6\linewidth}{!}{
% \resizebox{0.98\linewidth}{!}{
\begin{tabular}{lcccc|c}
    \toprule
    \textbf{Classes (IoU/CD)}     &  \textbf{eyeglasses}     &  \textbf{laptop}     &  \textbf{oven}    & \textbf{mean}\\    
    \midrule
    \textbf{Ours (2-view)} & / & / & / & / & / \\
    \bottomrule \\
  \end{tabular}}
\caption{\small{Mean voxel IoU for 3D shape reconstruction with 4 input views.}}
\label{tab:mv3d4v}
%\vspace{-0.7cm}
\end{table*}
